From Retrieval to Generation: Comparing Different Approaches

Knowledge-intensive tasks, particularly open-domain question answering (ODQA), document reranking, and retrieval-augmented language modeling, require a balance between retrieval accuracy and generative flexibility. Traditional retrieval models such as BM25 and Dense Passage Retrieval (DPR), efficiently retrieve from large corpora but often lack semantic depth. Generative models like GPT-4-o provide richer contextual understanding but face challenges in maintaining factual consistency. In this work, we conduct a systematic evaluation of retrieval-based, generation-based, and hybrid models, with a primary focus on their performance in ODQA and related retrieval-augmented tasks. Our results show that dense retrievers, particularly DPR, achieve strong performance in ODQA with a top-1 accuracy of 50.17\% on NQ, while hybrid models improve nDCG@10 scores on BEIR from 43.42 (BM25) to 52.59, demonstrating their strength in document reranking. Additionally, we analyze language modeling tasks using WikiText-103, showing that retrieval-based approaches like BM25 achieve lower perplexity compared to generative and hybrid methods, highlighting their utility in retrieval-augmented generation. By providing detailed comparisons and practical insights into the conditions where each approach excels, we aim to facilitate future optimizations in retrieval, reranking, and generative models for ODQA and related knowledge-intensive applications.

==> sections/backup_tables.tex <==




\begin{comment}

\begin{table*}[!ht]
%\addtolength{\tabcolsep}{-0.65pt}
%\small
\centering
\resizebox{1.0\textwidth}{!}{  % Resize the table to fit the page width
\setlength\tabcolsep{3pt}
\begin{tabular}{@{}l|c | ccc| ccc | ccc |ccc | ccc | ccc @{}}
\toprule
 & & \multicolumn{9}{c|}{\tf{LLama V3 8B}} & \multicolumn{9}{c}{\tf{LLama V3.1 8B}}\\

\multirow{3}{*}{\tf{Retriever} }& \multirow{3}{*}{\tf{\# Doc}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c|}{\tf{WebQ}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c}{\tf{WebQ}} \\



                    &  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con \\
\midrule
%-      &      -  &     &    &   &    &    &  &   &  & \\
%\midrule
\multirow{4}{*}{BM25 } &       R  &    14.90  &  26.68  & 19.91  & 42.10 & 56.90 & 50.11 &  10.23 & 24.95 & 16.92 & 12.82 & 27.14 & 20.27 & 40.13 &58.40 &51.40 & 9.25 & 24.92 & 17.22 \\



&       G  &  24.68   &  45.43   &  33.85 &  52.23 &66.86 & 59.61 & 15.45  & 45.34 &35.28  &21.49  & 44.92 &33.65 & 48.74 &66.27 &  58.68 & 14.51& 45.73 & 35.03\\




&       R+G  & 25.51 & 45.22 & 34.29 & 53.29  & 70.04 & 62.75 & 15.05 & 42.75 & 32.77  & 22.29&45.46 & 34.37&  49.69 & 70.45&  62.98 & 13.97 & 43.91&33.56\\



&       G+R  &  25.67 & 45.93 &  34.70 & 53.24 & 69.54& 62.34 & 15.00 & 44.09 & 33.56  & 23.29 &46.10 &34.93 & 50.29 & 70.50 & 63.00& 13.43 & 43.53 & 32.72 \\

&   UPR   & 23.49  & 41.02 & 31.55 &  &&  &  &  &   &  & & &  & & &  &  &  \\



&   RankGPT   & 28.44  & 42.73 & 34.01 & - &-& - &  &  &   &  & & & - &- &- &  &  &  \\



\midrule
\multirow{4}{*}{MSS} &       R  &  12.82 & 22.96 & 17.36 & 31.90 &44.27  & 37.75 &  7.38 & 18.9 &11.81  & 11.19 & 23.37 & 17.81 & 30.74 & 45.82 &38.91 & 6.88 & 19.30 & 12.40\\



&       G  & 24.95  &  45.82 & 34.15 &  51.69 &  66.58 & 59.22 & 15.84 &46.06 &35.77  &21.46 & 45.29 & 33.90 & 47.98& 65.57& 57.84 & 14.12 & 45.25 &45.25 \\




&       R+G  &  25.54 &   44.79 &33.96 & 51.39 &67.52 & 59.99 & 14.96 & 43.14 & 32.48 & 21.57 & 44.88 & 33.93 & 47.75& 68.22 & 60.41 & 14.46 & 44.46& 33.31 \\



&       G+R  &  25.31  & 45.34 & 34.43 & 51.81 &  67.72 & 60.12 &   15.20 &43.75  & 33.12 & 22.68 & 45.55 &34.68 & 48.75 & 68.02 & 60.27 & 13.43 & 44.14 &33.07\\

&   UPR   &   &  &  & &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT    &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\
    
\midrule
\multirow{4}{*}{Contriever}   &       R  &  15.29  & 27.36 & 20.99 & 36.25 &  49.52 &  49.52 &  10.67 & 28.28 &  20.22 &13.24 & 27.68 &  21.88 &35.29  & 50.96 &44.19 & 9.35 &28.71 & 20.32\\




&       G  &  24.70 &  46.02 & 34.48 & 51.48  &  66.44 & 59.03 & 15.89  & 45.59 &35.23  &21.32 & 45.53 & 34.04 &  48.39 &65.82 &58.03 &  14.61 &45.67 &34.84\\




&       R+G  & 25.59  & 45.28 & 34.32 & 51.78 & 67.90 & 60.45 &   15.10 & 43.49 & 32.87 &22.18 & 45.26 & 34.45 & 48.38 & 68.84 & 61.47& 13.87 &45.07 &33.80\\


&       G+R  &  25.70 & 46.07   & 35.04  & 52.07 &  68.21& 60.98 & 15.50  &  44.08 & 33.21 & 23.13 &46.18  & 35.12 & 48.91 & 68.32 & 60.82 & 13.87 & 44.87 &34.10\\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT     &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\

\midrule
\multirow{4}{*}{DPR}  &       R  &   28.08 & 45.40 & 36.37 & 45.88 & 61.24 & 54.58 &45.88 &  61.24 &  54.58 & 23.21 & 44.99 & 36.03 &43.62 & 62.61& 55.97 & 14.32 & 38.27 &28.98 \\


&       G  & 25.06 & 45.81 & 34.34 &  51.66  &  66.51 &59.08 &  51.66 &  66.51 & 59.08  &21.41 & 45.37 & 34.15 & 48.21&65.76 &57.96 & 14.76 & 45.32 &34.59\\


&       R+G  &  28.94 & 48.82 & 37.31 &   54.41 & 70.83 & 63.68 &  54.41& 70.83 & 63.68  &24.62 & 48.50 & 37.28 & 50.61 & 71.30 & 63.99 & 14.32 & 46.55 & 34.94 \\


&       G+R  &  28.14 & 48.87 & 37.03 & 54.50& 70.53 & 63.42 & 54.50 & 70.53& 63.42 &25.51 & 50.28 & 38.53 & 51.65 & 71.66 &64.30 &14.81 & 46.59& 35.23\\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT    &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\


\midrule
\multirow{4}{*}{MSS+DPR}&       R  &   28.17 & 46.72 & 37.00 &  47.69 & 63.66 & 57.08 & 47.69 &  63.66 & 57.08 & 23.68 & 46.70 &37.53 & 45.72 & 65.24 & 58.53 & 13.92 &38.97 & 29.67\\



&       G  &  24.73  &  45.46 & 33.85 & 51.64  &66.90 & 59.40& 51.64 & 66.90 &59.40 & 21.80 & 45.28 & 33.90 &  47.98 & 65.51 & 57.83 &14.27 &46.14 &35.03\\


&       R+G  &  29.41 &   49.73 & 38.25 &   54.53 &70.86  &63.82 & 54.53 & 70.86 &63.82 &24.09 & 48.80 & 37.34 & 50.72 & 71.67 & 64.35 & 14.96 &46.40 & 34.94\\


&       G+R  &  28.61 & 49.27 & 37.36 &  54.48 & 71.16  & 63.91& 54.48 & 71.16 & 63.91 & 25.54 &50.30 &38.61 & 52.20 & 72.19 & 64.86 & 14.76 &46.42 & 35.33\\


&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\

\bottomrule


\end{tabular}
}
\caption{
QA using First retrieve and first GENREAD document by GenRead and using LLama 3 8B as RAG
}
\label{tab:qa}
\end{table*}
\end{comment}

\begin{table*}[!ht]
%\addtolength{\tabcolsep}{-0.65pt}
%\small
\centering
\resizebox{1.0\textwidth}{!}{  % Resize the table to fit the page width
\setlength\tabcolsep{3pt}
\begin{tabular}{@{}l|c | ccc| ccc | ccc |ccc | ccc | ccc @{}}
\toprule
 & & \multicolumn{9}{c|}{\tf{LLama V3 8B}} & \multicolumn{9}{c}{\tf{LLama V3.1 8B}}\\

\multirow{3}{*}{\tf{Retriever} }& \multirow{3}{*}{\tf{\# Doc}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c|}{\tf{WebQ}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c}{\tf{WebQ}} \\

                    &  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con \\
\midrule
\multirow{4}{*}{BM25 } &       R  &    14.90  &  26.68  & 19.91  & 42.10 & 56.90 & 50.11 &  10.23 & 24.95 & 16.92 & 12.82 & 27.14 & 20.27 & 40.13 &58.40 &51.40 & 9.25 & 24.92 & 17.22 \\

&       G  &  24.68   &  45.43   &  33.85 &  52.23 &66.86 & 59.61 & 15.45  & 45.34 &35.28  &21.49  & 44.92 &33.65 & 48.74 &66.27 &  58.68 & 14.51& 45.73 & 35.03\\

&       R+G  & 25.51 & 45.22 & 34.29 & 53.29  & 70.04 & 62.75 & 15.05 & 42.75 & 32.77  & 22.29&45.46 & 34.37&  49.69 & 70.45&  62.98 & 13.97 & 43.91&33.56\\

&       G+R  &  25.67 & 45.93 &  34.70 & 53.24 & 69.54& 62.34 & 15.00 & 44.09 & 33.56  & 23.29 &46.10 &34.93 & 50.29 & 70.50 & 63.00& 13.43 & 43.53 & 32.72 \\

&   UPR   & 23.49  & 41.02 & 31.55 & 55.85 & 69.59 & 62.65 & 17.27 & 44.15 & 32.68 & 24.24 & 40.68 & 31.47 & 55.22 & 68.14 & 61.78 & 17.67 & 41.68 & 30.71 \\

&   RankGPT   & 28.45  & 42.73 & 34.02 & - & - & - & 19.73 & 40.57 & 29.82 & 26.65 & 40.89 & 32.44 & - & - & - & 18.55 & 37.92 & 28.10 \\

\midrule
\multirow{4}{*}{MSS} &       R  &  12.82 & 22.96 & 17.36 & 31.90 &44.27  & 37.75 &  7.38 & 18.9 &11.81  & 11.19 & 23.37 & 17.81 & 30.74 & 45.82 &38.91 & 6.88 & 19.30 & 12.40\\

&       G  & 24.95  &  45.82 & 34.15 &  51.69 &  66.58 & 59.22 & 15.84 &46.06 &35.77  &21.46 & 45.29 & 33.90 & 47.98& 65.57& 57.84 & 14.12 & 45.25 &45.25 \\

&       R+G  &  25.54 &   44.79 &33.96 & 51.39 &67.52 & 59.99 & 14.96 & 43.14 & 32.48 & 21.57 & 44.88 & 33.93 & 47.75& 68.22 & 60.41 & 14.46 & 44.46& 33.31 \\

&       G+R  &  25.31  & 45.34 & 34.43 & 51.81 &  67.72 & 60.12 &   15.20 &43.75  & 33.12 & 22.68 & 45.55 &34.68 & 48.75 & 68.02 & 60.27 & 13.43 & 44.14 &33.07\\

&   UPR   & 23.35  & 40.52 & 31.55 & 53.78 & 68.67 & 61.63 & 17.08 & 43.97 & 32.14 & 24.43 & 41.08 & 31.77 & 54.97 & 68.46 & 61.73 & 16.70 & 42.20 & 31.30 \\

&   RankGPT    & 28.17 & 41.67 & 33.21 & - & - & - & 19.05 & 39.33 & 29.58 & 25.84 & 39.07 & 31.41 & - & - & - & 17.37 & 36.38 & 27.21 \\

\midrule
\multirow{4}{*}{Contriever}   &       R  &  15.29  & 27.36 & 20.99 & 36.25 &  49.52 &  49.52 &  10.67 & 28.28 &  20.22 &13.24 & 27.68 &  21.88 &35.29  & 50.96 &44.19 & 9.35 &28.71 & 20.32\\

&       G  &  24.70 &  46.02 & 34.48 & 51.48  &  66.44 & 59.03 & 15.89  & 45.59 &35.23  &21.32 & 45.53 & 34.04 &  48.39 &65.82 &58.03 &  14.61 &45.67 &34.84\\

&       R+G  & 25.59  & 45.28 & 34.32 & 51.78 & 67.90 & 60.45 &   15.10 & 43.49 & 32.87 &22.18 & 45.26 & 34.45 & 48.38 & 68.84 & 61.47& 13.87 &45.07 &33.80\\

&       G+R  &  25.70 & 46.07   & 35.04  & 52.07 &  68.21& 60.98 & 15.50  &  44.08 & 33.21 & 23.13 &46.18  & 35.12 & 48.91 & 68.32 & 60.82 & 13.87 & 44.87 &34.10\\

&   UPR   & 23.24  & 41.01 & 31.61 & 53.48 & 68.70 & 61.82 & 17.32 & 44.11 & 32.97 & 24.21 & 40.99 & 31.63 & 55.71 & 68.74 & 61.98 & 17.62 & 37.73 & 28.44 \\

&   RankGPT     & 30.55  & 44.25 & 35.40 & - & - & - & 19.78 & 41.18 & 31.10 & 28.86 & 42.42 & 33.68 & - & - & - & 17.62 & 37.73 & 28.44 \\

\midrule
\multirow{4}{*}{DPR}  &       R  &   28.08 & 45.40 & 36.37 & 45.88 & 61.24 & 54.58 &45.88 &  61.24 &  54.58 & 23.21 & 44.99 & 36.03 &43.62 & 62.61& 55.97 & 14.32 & 38.27 &28.98 \\

&       G  & 25.06 & 45.81 & 34.34 &  51.66  &  66.51 &59.08 &  51.66 &  66.51 & 59.08  &21.41 & 45.37 & 34.15 & 48.21&65.76 &57.96 & 14.76 & 45.32 &34.59\\

&       R+G  &  28.94 & 48.82 & 37.31 &   54.41 & 70.83 & 63.68 &  54.41& 70.83 & 63.68  &24.62 & 48.50 & 37.28 & 50.61 & 71.30 & 63.99 & 14.32 & 46.55 & 34.94 \\

&       G+R  &  28.14 & 48.87 & 37.03 & 54.50& 70.53 & 63.42 & 54.50 & 70.53& 63.42 &25.51 & 50.28 & 38.53 & 51.65 & 71.66 &64.30 &14.81 & 46.59& 35.23\\

&   UPR   & 23.60  & 41.18 & 31.77 & 53.41 & 68.60 & 61.60 & 18.06 & 44.01 & 32.48 & 24.74 & 41.32 & 31.75 & 56.07 & 69.14 & 62.41 & 19.64 & 39.77 & 29.87 \\

&   RankGPT    & 31.74 & 46.41 & 36.76 & - & - & - & 20.42 & 40.84 & 31.00 & 29.58 & 43.92 & 34.65 & - & - & - & 19.64 & 39.77 & 29.87 \\

\midrule
\multirow{4}{*}{MSS+DPR}&       R  &   28.17 & 46.72 & 37.00 &  47.69 & 63.66 & 57.08 & 47.69 &  63.66 & 57.08 & 23.68 & 46.70 &37.53 & 45.72 & 65.24 & 58.53 & 13.92 &38.97 & 29.67\\

&       G  &  24.73  &  45.46 & 33.85 & 51.64  &66.90 & 59.40& 51.64 & 66.90 &59.40 & 21.80 & 45.28 & 33.90 &  47.98 & 65.51 & 57.83 &14.27 &46.14 &35.03\\

&       R+G  &  29.41 &   49.73 & 38.25 &   54.53 &70.86  &63.82 & 54.53 & 70.86 &63.82 &24.09 & 48.80 & 37.34 & 50.72 & 71.67 & 64.35 & 14.96 &46.40 & 34.94\\

&       G+R  &  28.61 & 49.27 & 37.36 &  54.48 & 71.16  & 63.91& 54.48 & 71.16 & 63.91 & 25.54 &50.30 &38.61 & 52.20 & 72.19 & 64.86 & 14.76 &46.42 & 35.33\\

&   UPR   & 23.10  & 40.81 & 31.25 & 53.65 & 68.61 & 61.69 & 16.68 & 44.07 & 32.48 & 25.24 & 41.17 & 31.83 & 55.52 & 68.76 & 61.90 & 18.99 & 40.76 & 30.22 \\

&   RankGPT   & 31.94 & 45.95 & 36.59 & - & - & - & 21.41 & 42.54 & 32.14 & 29.95 & 45.00 & 36.49 & - & - & - & 18.99 & 40.76 & 30.22 \\

\bottomrule
\end{tabular}
}
\caption{QA using First retrieve and first GENREAD document by GenRead and using LLama 3 8B as RAG}
\label{tab:qa}
\end{table*}


\begin{comment}
\begin{table*}[!ht]
%\addtolength{\tabcolsep}{-0.65pt}
%\small
\centering
\resizebox{1.0\textwidth}{!}{  % Resize the table to fit the page width
\setlength\tabcolsep{3pt}
\begin{tabular}{@{}l|c | ccc| ccc | ccc |ccc | ccc | ccc @{}}
\toprule
 & & \multicolumn{9}{c|}{\tf{Gemma-2-2b}} & \multicolumn{9}{c}{\tf{Gemma-2-9b}}\\

\multirow{3}{*}{\tf{Retriever} }& \multirow{3}{*}{\tf{\# Doc}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c|}{\tf{WebQ}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c}{\tf{WebQ}} \\

&  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con \\
\midrule

\multirow{3}{*}{BM25 } &       R   & 14.02 & 25.55 & 18.53 & 43.28 & 52.78 & 47.01 & 14.71 & 37.74 & 27.21 & 19.81 & 26.95 & 22.05 & 57.55 & 65.53 & 60.29 & 14.96 & 24.87 & 20.13 \\

&       G   & 27.01 & 46.85 & 35.35 & 59.91 & 72.99 & 66.36 & 19.34 & 50.19 & 38.93 & 28.28 & 46.46 & 36.04 & 63.02 & 75.33 & 68.83 & 18.65 & 50.57 & 39.37 \\

&       R+G   & 28.39 & 46.41 & 35.62 & 59.89 & 73.39 & 66.53 & 19.29 & 47.44 & 35.93 & 28.45 & 45.09 & 35.54 & 63.50 & 75.23 & 68.50 & 19.05 & 45.38 & 34.94 \\

&       G+R   & 28.50 & 46.50 & 35.68 & 59.87 & 72.99 & 66.21 & 19.73 & 48.22 & 36.47 & 28.42 & 45.67 & 35.96 & 62.94 & 75.44 & 68.64 & 19.34 & 45.83 & 35.53 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\

\midrule
\multirow{4}{*}{MSS} &       R   & 13.96 & 25.41 & 18.50 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

&       G   & 27.06 & 46.87 & 35.29 & 59.27 & 72.32 & 65.49 & 19.34 & 50.19 & 38.93 & 27.95 & 46.77 & 36.01 & 62.67 & 74.93 & 68.41 & 18.65 & 50.57 & 39.37 \\

&       R+G   & 28.48 & 46.36 & 35.48 & 58.63 & 71.48 & 64.65 & 19.29 & 47.05 & 35.78 & 28.56 & 45.27 & 35.65 & 62.53 & 73.97 & 67.27 & 18.80 & 44.44 & 34.01 \\

&       G+R   & 28.42 & 46.18 & 35.57 & 58.47 & 71.27 & 64.46 & 19.78 & 47.79 & 36.07 & 28.31 & 45.53 & 35.37 & 61.78 & 73.76 & 67.07 & 18.55 & 45.11 & 35.09 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\

\midrule
\multirow{4}{*}{Contriever}   &       R   & 13.96 & 25.41 & 18.50 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

&       G   & 27.06 & 46.87 & 35.29 & 59.27 & 72.32 & 65.49 & 19.34 & 50.19 & 38.93 & 27.95 & 46.77 & 36.01 & 62.67 & 74.93 & 68.41 & 18.65 & 50.57 & 39.37 \\

&       R+G   & 28.78 & 46.98 & 36.12 & 58.86 & 71.68 & 64.81 & 20.28 & 48.42 & 37.30 & 28.84 & 45.33 & 35.90 & 62.85 & 73.89 & 67.21 & 19.64 & 46.01 & 35.43 \\

&       G+R   & 28.75 & 46.70 & 35.98 & 58.64 & 71.33 & 64.57 & 20.13 & 48.24 & 36.86 & 28.37 & 45.46 & 36.07 & 61.97 & 73.87 & 67.07 & 19.09 & 45.95 & 36.17 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\

\midrule
\multirow{4}{*}{DPR}  &       R   & 13.99 & 25.44 & 18.53 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

&       G  & 27.06 & 46.87 & 35.29 & 59.27 & 72.32 & 65.49 & 19.34 & 50.19 & 38.93 & 27.92 & 46.75 & 35.98 & 62.67 & 74.93 & 68.41 & 18.65 & 50.57 & 39.37 \\

&       R+G   & 30.25 & 48.89 & 37.73 & 60.16 & 73.19 & 66.28 & 20.18 & 48.36 & 36.66 & 30.83 & 47.93 & 37.89 & 63.72 & 74.99 & 68.27 & 19.93 & 46.16 & 35.88 \\

&       G+R   & 30.72 & 48.78 & 37.45 & 60.17 & 72.98 & 66.22 & 20.52 & 48.93 & 36.86 & 29.92 & 47.48 & 37.12 & 63.18 & 75.00 & 68.29 & 19.39 & 46.59 & 36.32 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\

\midrule
\multirow{4}{*}{MSS+DPR}&       R   & 13.96 & 25.41 & 18.50 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

&       G   & 27.06 & 46.87 & 35.29 & 59.27 & 72.32 & 65.49 & 19.34 & 50.19 & 38.93 & 28.25 & 46.47 & 36.01 & 62.67 & 74.93 & 68.41 & 18.60 & 46.85 & 36.32 \\

&       R+G   & 30.91 & 49.23 & 38.12 & 60.56 & 73.67 & 66.82 & 20.72 & 48.67 & 36.91 & 30.58 & 47.85 & 37.73 & 63.76 & 75.20 & 68.48 & 19.93 & 46.62 & 36.32 \\

&       G+R  & 30.66 & 49.15 & 37.98 & 60.25 & 73.53 & 66.68 & 21.26 & 49.67 & 37.70 & 29.94 & 47.61 & 37.40 & 63.17 & 75.19 & 68.37 & 20.13 & 46.90 & 37.01 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\

\bottomrule
\end{tabular}
}
\caption{
QA using First retrieve and first GENREAD document by GenRead and using  as RAG
}
\label{tab:qa}
\end{table*}

\end{comment}




\begin{table*}[!ht]
%\addtolength{\tabcolsep}{-0.65pt}
%\small
\centering
\resizebox{1.0\textwidth}{!}{  % Resize the table to fit the page width
\setlength\tabcolsep{3pt}
\begin{tabular}{@{}l|c | ccc| ccc | ccc |ccc | ccc | ccc @{}}
\toprule
 & & \multicolumn{9}{c|}{\tf{Gemma-2-2b}} & \multicolumn{9}{c}{\tf{Gemma-2-9b}}\\

\multirow{3}{*}{\tf{Retriever} }& \multirow{3}{*}{\tf{\# Doc}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c|}{\tf{WebQ}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c}{\tf{WebQ}} \\

&  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con \\
\midrule

\multirow{6}{*}{BM25 } &       R   & 14.02 & 25.55 & 18.53 & 43.28 & 52.78 & 47.01 & 14.71 & 37.74 & 27.21 & 19.81 & 26.95 & 22.05 & 57.55 & 65.53 & 60.29 & 14.96 & 24.87 & 20.13 \\

&       G   & 27.01 & 46.85 & 35.35 & 59.91 & 72.99 & 66.36 & 19.34 & 50.19 & 38.93 & 28.28 & 46.46 & 36.04 & 63.02 & 75.33 & 68.83 & 18.65 & 50.57 & 39.37 \\

&       R+G   & 28.39 & 46.41 & 35.62 & 59.89 & 73.39 & 66.53 & 19.29 & 47.44 & 35.93 & 28.45 & 45.09 & 35.54 & 63.50 & 75.23 & 68.50 & 19.05 & 45.38 & 34.94 \\

&       G+R   & 28.50 & 46.50 & 35.68 & 59.87 & 72.99 & 66.21 & 19.73 & 48.22 & 36.47 & 28.42 & 45.67 & 35.96 & 62.94 & 75.44 & 68.64 & 19.34 & 45.83 & 35.53 \\

&   UPR   & 26.23 & 44.37 & 33.99 & 58.71 & 71.59 & 64.79 & 19.78 & 48.16 & 36.47 & 23.41 & 41.52 & 32.24 & 58.74 & 71.92 & 65.20 & 15.94 & 46.16 & 34.15 \\

&   RankGPT   & 30.36 & 45.96 & 36.09 & - & - & - & 21.11 & 45.13 & 34.35 & 30.75 & 43.48 & 35.46 & - & - & - & 21.06 & 39.32 & 31.15 \\

\midrule
\multirow{6}{*}{MSS} &       R   & 13.96 & 25.41 & 18.50 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

&       G   & 27.06 & 46.87 & 35.29 & 59.27 & 72.32 & 65.49 & 19.34 & 50.19 & 38.93 & 27.95 & 46.77 & 36.01 & 62.67 & 74.93 & 68.41 & 18.65 & 50.57 & 39.37 \\

&       R+G   & 28.48 & 46.36 & 35.48 & 58.63 & 71.48 & 64.65 & 19.29 & 47.05 & 35.78 & 28.56 & 45.27 & 35.65 & 62.53 & 73.97 & 67.27 & 18.80 & 44.44 & 34.01 \\

&       G+R   & 28.42 & 46.18 & 35.57 & 58.47 & 71.27 & 64.46 & 19.78 & 47.79 & 36.07 & 28.31 & 45.53 & 35.37 & 61.78 & 73.76 & 67.07 & 18.55 & 45.11 & 35.09 \\

&   UPR   & 26.20 & 44.14 & 33.77 & 58.15 & 71.02 & 64.10 & 19.73 & 48.92 & 36.96 & 23.10 & 41.49 & 32.05 & 57.50 & 71.15 & 64.33 & 15.85 & 47.20 & 34.65 \\

&   RankGPT   & 29.17 & 45.00 & 35.32 & - & - & - & 19.93 & 44.61 & 34.10 & 29.97 & 42.59 & 34.85 & - & - & - & 19.64 & 36.91 & 29.72 \\

\midrule
\multirow{6}{*}{Contriever}   &       R   & 13.96 & 25.41 & 18.50 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

&       G   & 27.06 & 46.87 & 35.29 & 59.27 & 72.32 & 65.49 & 19.34 & 50.19 & 38.93 & 27.95 & 46.77 & 36.01 & 62.67 & 74.93 & 68.41 & 18.65 & 50.57 & 39.37 \\

&       R+G   & 28.78 & 46.98 & 36.12 & 58.86 & 71.68 & 64.81 & 20.28 & 48.42 & 37.30 & 28.84 & 45.33 & 35.90 & 62.85 & 73.89 & 67.21 & 19.64 & 46.01 & 35.43 \\

&       G+R   & 28.75 & 46.70 & 35.98 & 58.64 & 71.33 & 64.57 & 20.13 & 48.24 & 36.86 & 28.37 & 45.46 & 36.07 & 61.97 & 73.87 & 67.07 & 19.09 & 45.95 & 36.17 \\

&   UPR   & 26.26 & 44.26 & 33.82 & 58.37 & 71.17 & 64.23 & 19.83 & 48.32 & 36.61 & 23.21 & 41.46 & 32.08 & 57.64 & 71.20 & 64.36 & 16.14 & 46.12 & 34.01 \\

&   RankGPT   & 32.11 & 47.86 & 38.31 & - & - & - & 20.67 & 45.77 & 34.89 & 32.44 & 44.83 & 36.79 & - & - & - & 19.88 & 38.57 & 30.02 \\

\midrule
\multirow{6}{*}{DPR}  &       R   & 13.99 & 25.44 & 18.53 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

&       G  & 27.06 & 46.87 & 35.29 & 59.27 & 72.32 & 65.49 & 19.34 & 50.19 & 38.93 & 27.92 & 46.75 & 35.98 & 62.67 & 74.93 & 68.41 & 18.65 & 50.57 & 39.37 \\

&       R+G   & 30.25 & 48.89 & 37.73 & 60.16 & 73.19 & 66.28 & 20.18 & 48.36 & 36.66 & 30.83 & 47.93 & 37.89 & 63.72 & 74.99 & 68.27 & 19.93 & 46.16 & 35.88 \\

&       G+R   & 30.72 & 48.78 & 37.45 & 60.17 & 72.98 & 66.22 & 20.52 & 48.93 & 36.86 & 29.92 & 47.48 & 37.12 & 63.18 & 75.00 & 68.29 & 19.39 & 46.59 & 36.32 \\

&   UPR   & 26.51 & 44.62 & 34.16 & 58.71 & 71.72 & 64.78 & 19.78 & 48.62 & 36.86 & 23.38 & 41.80 & 32.38 & 57.85 & 71.54 & 64.75 & 16.04 & 46.56 & 34.50 \\

&   RankGPT   & 34.16 & 50.26 & 39.42 & - & - & - & 21.21 & 46.41 & 35.48 & 34.04 & 47.14 & 38.64 & - & - & - & 21.01 & 40.41 & 31.69 \\

\midrule
\multirow{6}{*}{MSS+DPR}&       R   & 13.96 & 25.41 & 18.50 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

&       G   & 27.06 & 46.87 & 35.29 & 59.27 & 72.32 & 65.49 & 19.34 & 50.19 & 38.93 & 28.25 & 46.47 & 36.01 & 62.67 & 74.93 & 68.41 & 18.60 & 46.85 & 36.32 \\

&       R+G   & 30.91 & 49.23 & 38.12 & 60.56 & 73.67 & 66.82 & 20.72 & 48.67 & 36.91 & 30.58 & 47.85 & 37.73 & 63.76 & 75.20 & 68.48 & 19.93 & 46.62 & 36.32 \\

&       G+R  & 30.66 & 49.15 & 37.98 & 60.25 & 73.53 & 66.68 & 21.26 & 49.67 & 37.70 & 29.94 & 47.61 & 37.40 & 63.17 & 75.19 & 68.37 & 20.13 & 46.90 & 37.01 \\

&   UPR   & 26.54 & 44.67 & 34.21 & 58.64 & 71.50 & 64.55 & 19.49 & 48.03 & 36.02 & 23.46 & 41.75 & 32.38 & 57.75 & 71.34 & 64.48 & 15.94 & 45.96 & 33.56 \\

&   RankGPT   & 32.51 & 49.77 & 39.53 & - & - & - & 21.41 & 47.58 & 36.52 & 32.13 & 46.55 & 38.29 & - & - & - & 21.06 & 40.72 & 32.04 \\

\bottomrule
\end{tabular}
}
\caption{
QA using First retrieve and first GENREAD document by GenRead and using Gemma-2 models as RAG
}
\label{tab:qa}
\end{table*}




\begin{comment}

\begin{table*}[!ht]
%\addtolength{\tabcolsep}{-0.65pt}
%\small
\centering
\resizebox{1.0\textwidth}{!}{  % Resize the table to fit the page width
\setlength\tabcolsep{3pt}
\begin{tabular}{@{}l|c | ccc| ccc | ccc |ccc | ccc | ccc @{}}
\toprule
 & & \multicolumn{9}{c|}{\tf{Llama-2-13b-hf}} & \multicolumn{9}{c}{\tf{Mistral-7B-v0.1}}\\

\multirow{3}{*}{\tf{Retriever} }& \multirow{3}{*}{\tf{\# Doc}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c|}{\tf{WebQ}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c}{\tf{WebQ}} \\



                    &  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con \\
\midrule
%-      &      -  &     &    &   &    &    &  &   &  & \\
%\midrule
\multirow{3}{*}{BM25 } 
&       R   & 21.14 & 30.82 & 24.46 & 57.90 & 65.27 & 59.57 & 19.54 & 37.38 & 27.51 & 11.19 & 13.45 & 11.80 & 52.85 & 58.11 & 53.82 & 6.40 & 8.46 & 6.84 \\

&       G   & 28.06 & 44.60 & 34.21 & 62.64 & 73.63 & 67.13 & 20.32 & 45.54 & 34.40 & 27.01 & 41.30 & 32.19 & 62.64 & 72.63 & 66.19 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 26.62 & 41.96 & 32.47 & 61.35 & 73.01 & 66.34 & 19.00 & 43.61 & 32.53 & 25.68 & 37.68 & 30.11 & 60.45 & 69.76 & 63.49 & 15.65 & 29.42 & 22.54 \\

&       G+R   & 26.79 & 43.16 & 33.35 & 62.01 & 73.14 & 66.67 & 19.24 & 43.70 & 32.68 & 23.71 & 34.64 & 27.87 & 58.56 & 67.61 & 61.63 & 13.44 & 26.74 & 20.08 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\
\midrule
\multirow{4}{*}{MSS} 
&       R   & 21.52 & 30.92 & 24.18 & 51.75 & 58.58 & 53.35 & 20.62 & 39.45 & 29.68 & 11.08 & 13.33 & 11.66 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\

&       G   & 28.01 & 43.22 & 33.74 & 60.66 & 72.01 & 65.43 & 19.44 & 44.80 & 34.20 & 27.15 & 41.40 & 32.19 & 61.28 & 71.06 & 64.71 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 26.81 & 42.48 & 33.02 & 58.64 & 70.39 & 63.87 & 19.05 & 42.74 & 32.14 & 25.90 & 38.34 & 30.58 & 56.28 & 64.82 & 59.03 & 14.57 & 27.91 & 20.96 \\

&       G+R   & 27.48 & 43.97 & 33.88 & 59.56 & 71.14 & 64.63 & 18.75 & 42.48 & 31.64 & 23.10 & 33.75 & 27.26 & 52.15 & 59.83 & 54.59 & 13.09 & 24.77 & 18.31 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\
\midrule
\multirow{4}{*}{Contriever}   
&       R   & 20.47 & 30.13 & 23.85 & 42.69 & 47.12 & 43.40 & 19.98 & 37.74 & 27.61 & 11.08 & 13.33 & 11.66 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\

&       G   & 26.79 & 43.16 & 33.35 & 61.28 & 71.06 & 64.71 & 19.69 & 44.88 & 33.76 & 27.15 & 41.40 & 32.19 & 61.28 & 71.06 & 64.71 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 27.45 & 42.89 & 33.27 & 56.43 & 65.00 & 59.20 & 19.59 & 43.25 & 32.19 & 25.35 & 37.57 & 30.08 & 56.43 & 65.00 & 59.20 & 15.31 & 27.88 & 20.82 \\

&       G+R   & 27.17 & 43.64 & 33.74 & 52.66 & 60.52 & 55.33 & 19.88 & 44.21 & 33.61 & 23.02 & 33.53 & 27.29 & 54.39 & 62.52 & 57.18 & 13.44 & 25.79 & 19.24 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\
\midrule
\multirow{4}{*}{DPR}  
&       R   & 21.94 & 31.36 & 24.88 & 51.07 & 57.97 & 52.71 & 19.83 & 37.35 & 28.05 & 11.11 & 13.36 & 11.69 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\

&       G  & 28.12 & 44.10 & 34.32 & 60.85 & 71.87 & 65.44 & 20.47 & 45.05 & 34.15 & 27.15 & 41.40 & 32.19 & 61.28 & 71.06 & 64.71 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 28.81 & 44.73 & 34.82 & 58.00 & 67.03 & 61.14 & 20.32 & 45.14 & 34.25 & 27.70 & 40.40 & 32.47 & 58.00 & 67.03 & 61.14 & 16.44 & 32.14 & 24.31 \\

&       G+R   & 27.92 & 44.15 & 34.27 & 60.01 & 71.44 & 64.93 & 20.72 & 45.02 & 34.15 & 25.01 & 35.90 & 29.06 & 54.64 & 62.57 & 57.27 & 14.71 & 28.39 & 21.75 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\
\midrule
\multirow{4}{*}{MSS+DPR}
&       R   & 21.47 & 31.26 & 24.60 & 51.35 & 58.26 & 53.01 & 19.83 & 37.37 & 27.61 & 11.08 & 13.33 & 11.66 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\

&       G   & 28.20 & 43.75 & 34.07 & 60.44 & 71.60 & 65.09 & 20.13 & 45.50 & 34.30 & 27.15 & 41.40 & 32.19 & 61.28 & 71.06 & 64.71 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 28.45 & 45.21 & 35.21 & 59.50 & 71.17 & 64.79 & 19.78 & 44.57 & 33.46 & 27.40 & 39.95 & 31.94 & 58.03 & 67.43 & 61.49 & 16.44 & 31.62 & 23.97 \\

&       G+R  & 28.73 & 44.67 & 34.79 & 59.96 & 71.90 & 65.57 & 20.77 & 45.09 & 34.10 & 25.07 & 35.95 & 28.92 & 54.39 & 62.52 & 57.18 & 14.96 & 29.13 & 22.00 \\

&   UPR   &   &  &  &  &&  &  &  &   &  & & &  & & &  &  &  \\
&   RankGPT   &   &  &  & - &-&-  &  &  &   &  & & & - &- & -&  &  &  \\
\bottomrule
\end{tabular}
}
\caption{
QA using First retrieve and first GENREAD document by GenRead and using Llama-2-13b-hf and Mistral-7B-v0.1 as RAG
}
\label{tab:qa}
\end{table*}
\end{comment}

\begin{table*}[!ht]
%\addtolength{\tabcolsep}{-0.65pt}
%\small
\centering
\resizebox{1.0\textwidth}{!}{  % Resize the table to fit the page width
\setlength\tabcolsep{3pt}
\begin{tabular}{@{}l|c | ccc| ccc | ccc |ccc | ccc | ccc @{}}
\toprule
 & & \multicolumn{9}{c|}{\tf{Llama-2-13b-hf}} & \multicolumn{9}{c}{\tf{Mistral-7B-v0.1}}\\

\multirow{3}{*}{\tf{Retriever} }& \multirow{3}{*}{\tf{\# Doc}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c|}{\tf{WebQ}} & \multicolumn{3}{c}{\tf{NQ}} & \multicolumn{3}{c}{\tf{TriviaQA}} & \multicolumn{3}{c}{\tf{WebQ}} \\

&  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con \\
\midrule

\multirow{6}{*}{BM25 } 
&       R   & 21.14 & 30.82 & 24.46 & 57.90 & 65.27 & 59.57 & 19.54 & 37.38 & 27.51 & 11.19 & 13.45 & 11.80 & 52.85 & 58.11 & 53.82 & 6.40 & 8.46 & 6.84 \\

&       G   & 28.06 & 44.60 & 34.21 & 62.64 & 73.63 & 67.13 & 20.32 & 45.54 & 34.40 & 27.01 & 41.30 & 32.19 & 62.64 & 72.63 & 66.19 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 26.62 & 41.96 & 32.47 & 61.35 & 73.01 & 66.34 & 19.00 & 43.61 & 32.53 & 25.68 & 37.68 & 30.11 & 60.45 & 69.76 & 63.49 & 15.65 & 29.42 & 22.54 \\

&       G+R   & 26.79 & 43.16 & 33.35 & 62.01 & 73.14 & 66.67 & 19.24 & 43.70 & 32.68 & 23.71 & 34.64 & 27.87 & 58.56 & 67.61 & 61.63 & 13.44 & 26.74 & 20.08 \\

&   UPR   & 27.59 & 42.65 & 32.99 & 61.60 & 71.62 & 65.00 & 20.37 & 44.09 & 33.76 & 25.18 & 40.47 & 31.11 & 59.64 & 69.91 & 63.20 & 17.18 & 40.89 & 30.46 \\

&   RankGPT   & 29.22 & 43.00 & 34.21 & - & - & - & 21.99 & 41.25 & 31.15 & 25.35 & 40.47 & 31.36 & - & - & - & 17.18 & 40.90 & 30.46 \\

\midrule
\multirow{6}{*}{MSS} 
&       R   & 21.52 & 30.92 & 24.18 & 51.75 & 58.58 & 53.35 & 20.62 & 39.45 & 29.68 & 11.08 & 13.33 & 11.66 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\

&       G   & 28.01 & 43.22 & 33.74 & 60.66 & 72.01 & 65.43 & 19.44 & 44.80 & 34.20 & 27.15 & 41.40 & 32.19 & 61.28 & 71.06 & 64.71 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 26.81 & 42.48 & 33.02 & 58.64 & 70.39 & 63.87 & 19.05 & 42.74 & 32.14 & 25.90 & 38.34 & 30.58 & 56.28 & 64.82 & 59.03 & 14.57 & 27.91 & 20.96 \\

&       G+R   & 27.48 & 43.97 & 33.88 & 59.56 & 71.14 & 64.63 & 18.75 & 42.48 & 31.64 & 23.10 & 33.75 & 27.26 & 52.15 & 59.83 & 54.59 & 13.09 & 24.77 & 18.31 \\

&   UPR   & 27.29 & 42.28 & 32.63 & 59.23 & 69.93 & 63.56 & 20.72 & 44.50 & 33.96 & 23.77 & 40.41 & 30.97 & 57.24 & 67.67 & 61.04 & 17.42 & 42.17 & 31.20 \\

&   RankGPT   & 27.56 & 41.77 & 33.05 & - & - & - & 20.77 & 44.50 & 33.96 & 23.77 & 39.08 & 29.28 & - & - & - & 16.98 & 39.87 & 29.43 \\

\midrule
\multirow{6}{*}{Contriever}   
&       R   & 20.47 & 30.13 & 23.85 & 42.69 & 47.12 & 43.40 & 19.98 & 37.74 & 27.61 & 11.08 & 13.33 & 11.66 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\

&       G   & 26.79 & 43.16 & 33.35 & 61.28 & 71.06 & 64.71 & 19.69 & 44.88 & 33.76 & 27.15 & 41.40 & 32.19 & 61.28 & 71.06 & 64.71 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 27.45 & 42.89 & 33.27 & 56.43 & 65.00 & 59.20 & 19.59 & 43.25 & 32.19 & 25.35 & 37.57 & 30.08 & 56.43 & 65.00 & 59.20 & 15.31 & 27.88 & 20.82 \\

&       G+R   & 27.17 & 43.64 & 33.74 & 52.66 & 60.52 & 55.33 & 19.88 & 44.21 & 33.61 & 23.02 & 33.53 & 27.29 & 54.39 & 62.52 & 57.18 & 13.44 & 25.79 & 19.24 \\

&   UPR   & 26.57 & 41.99 & 32.44 & 59.60 & 70.02 & 63.58 & 20.72 & 44.65 & 33.56 & 25.10 & 40.43 & 31.02 & 57.26 & 67.63 & 61.11 & 17.27 & 40.48 & 29.97 \\

&   RankGPT   & 30.39 & 44.60 & 36.09 & - & - & - & 20.72 & 44.65 & 33.56 & 25.10 & 40.48 & 31.02 & - & - & - & 17.27 & 40.48 & 29.97 \\

\midrule
\multirow{6}{*}{DPR}  
&       R   & 21.94 & 31.36 & 24.88 & 51.07 & 57.97 & 52.71 & 19.83 & 37.35 & 28.05 & 11.11 & 13.36 & 11.69 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\

&       G  & 28.12 & 44.10 & 34.32 & 60.85 & 71.87 & 65.44 & 20.47 & 45.05 & 34.15 & 27.15 & 41.40 & 32.19 & 61.28 & 71.06 & 64.71 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 28.81 & 44.73 & 34.82 & 58.00 & 67.03 & 61.14 & 20.32 & 45.14 & 34.25 & 27.70 & 40.40 & 32.47 & 58.00 & 67.03 & 61.14 & 16.44 & 32.14 & 24.31 \\

&       G+R   & 27.92 & 44.15 & 34.27 & 60.01 & 71.44 & 64.93 & 20.72 & 45.02 & 34.15 & 25.01 & 35.90 & 29.06 & 54.64 & 62.57 & 57.27 & 14.71 & 28.39 & 21.75 \\

&   UPR   & 27.45 & 42.93 & 33.02 & 60.05 & 70.49 & 63.96 & 20.62 & 44.81 & 33.91 & 25.26 & 40.71 & 31.36 & 57.53 & 67.80 & 61.31 & 17.18 & 41.20 & 30.66 \\

&   RankGPT   & 32.77 & 47.56 & 38.06 & - & - & - & 22.15 & 44.37 & 33.81 & 25.26 & 40.71 & 31.36 & - & - & - & 17.18 & 41.20 & 30.66 \\

\midrule
\multirow{6}{*}{MSS+DPR}
&       R   & 21.47 & 31.26 & 24.60 & 51.35 & 58.26 & 53.01 & 19.83 & 37.37 & 27.61 & 11.08 & 13.33 & 11.66 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\

&       G   & 28.20 & 43.75 & 34.07 & 60.44 & 71.60 & 65.09 & 20.13 & 45.50 & 34.30 & 27.15 & 41.40 & 32.19 & 61.28 & 71.06 & 64.71 & 16.09 & 33.01 & 24.70 \\

&       R+G   & 28.45 & 45.21 & 35.21 & 59.50 & 71.17 & 64.79 & 19.78 & 44.57 & 33.46 & 27.40 & 39.95 & 31.94 & 58.03 & 67.43 & 61.49 & 16.44 & 31.62 & 23.97 \\

&       G+R  & 28.73 & 44.67 & 34.79 & 59.96 & 71.90 & 65.57 & 20.77 & 45.09 & 34.10 & 25.07 & 35.95 & 28.92 & 54.39 & 62.52 & 57.18 & 14.96 & 29.13 & 22.00 \\

&   UPR   & 27.45 & 42.91 & 33.10 & 60.00 & 71.52 & 64.07 & 19.98 & 44.81 & 33.32 & 25.24 & 40.59 & 31.25 & 57.47 & 67.80 & 61.12 & 16.09 & 44.33 & 33.32 \\

&   RankGPT   & 32.61 & 48.90 & 40.19 & - & - & - & 21.95 & 43.73 & 33.32 & 25.24 & 40.59 & 31.25 & - & - & - & 16.09 & 44.33 & 33.32 \\

\bottomrule
\end{tabular}
}
\caption{
QA using First retrieve and first GENREAD document by GenRead and using Llama-2-13b-hf and Mistral-7B-v0.1 as RAG
}
\label{tab:qa}
\end{table*}

